VSE++: Improving Visual-Semantic Embeddings with Hard Negatives

We present a new technique for learning visual-semantic embeddings for cross-modal retrieval. Inspired by hard negative mining, the use of hard negatives in structured prediction, and ranking loss functions, we introduce a simple change to common loss functions used for multi-modal embeddings. That, combined with fine-tuning and use of augmented data, yields significant gains in retrieval performance. We showcase our approach, VSE++, on MS-COCO and Flickr30K datasets, using ablation studies and comparisons with existing methods. On MS-COCO our approach outperforms state-of-the-art methods by 8.8% in caption retrieval and 11.3% in image retrieval (at R@1).

==> neg_size.tex <==

\subsection{Effect of Negative Set Size on \MAX{} Loss}

\begin{figure*}[htb!]
    % \begin{tabular}{>{\centering\arraybackslash}m{.47\linewidth}
    %     >{\centering\arraybackslash}m{.47\linewidth}}
    \begin{subfigure}[b]{.47\textwidth}
        \includegraphics[width=\linewidth]{images/sum_vs_max_f30k.png}
        \caption{}\label{fig:sum_vs_max}
    \end{subfigure}
        \hfill
    \begin{subfigure}[b]{.47\textwidth}
        % &
        \includegraphics[width=\linewidth]{images/neg_size_recall.png}
    \caption{}\label{fig:neg_size}
    % \end{tabular}
    \end{subfigure}
        \caption{Analysis of the behavior of the \MAX{} loss on the \fthk{} 
        dataset training with \RC{}. Fig.~\subref{fig:sum_vs_max} compares the 
        \SUM{} loss to the \MAX{} loss (Table~\ref{tb:f30k}, 
        row~\ref{f30k:VSEzRC} and row~\ref{f30k:VSEppRC}). Notice that, in the 
        first $5$ epochs the \SUM{} loss achieves a better performance, 
        however, from there-on the \MAX{} loss leads to much higher recall 
        rates.  Fig.~\subref{fig:neg_size} shows the effect of the negative set 
        size on the R@$1$ performance.}
        \label{fig:svm_neg}
\end{figure*}

In practice, our \MAX{} loss searches for the hardest negative only 
within each mini-batch at each iteration. To explore the impact of this 
approximation we examined how performance depends on the effective 
sample size over which we searched for negatives (while keeping the mini-batch 
size fixed at $128$). In the extreme case, when the negative set is the 
training set, we get the hardest negatives in the entire training set.  As 
discussed in Sec.~\ref{sec:hard_neg}, sampling a negative set smaller than the 
training set can potentially be more robust to label errors.


% \begin{figure*}[htb!]
%     % \begin{tabular}{>{\centering\arraybackslash}m{.47\linewidth}
%     %     >{\centering\arraybackslash}m{.47\linewidth}}
%     \begin{subfigure}[b]{.47\textwidth}
%          \includegraphics[width=\linewidth]{images/sum_vs_max_vse.png}
%     \caption{}\label{fig:svm}
%     \end{subfigure}
%     \begin{subfigure}[b]{.47\textwidth}
%         % &
%         \includegraphics[width=\linewidth]{images/nonzero.png}
%         \caption{}\label{fig:nonzero}
%    \end{subfigure}
%     % \end{tabular}
%         \captionof{figure}{Comparison between the recall performance on the 
%         validation set of \coco{} for the \MAX{} loss and the \SUM{} loss.  
%         Fig.~\subref{fig:svm1}  compares \VSEz{} and \VSEpp{} with ResNet152 as 
%         the image encoder with/without fine-tuning (Table~\ref{tb:coco}, 
%         row~\ref{coco:VSEppRes} and row~\ref{coco:VSEppResFt} compared to 
%         Table~\ref{tb:vse0}, row~\ref{coco:VSEzRes} and 
%         row~\ref{coco:VSEzResFt}).  }
% \end{figure*}

% \david{Was the negative set always a subset of the mini-batch
% negatives when it's size was less than 128? When it's larger than 128 
% this cannot be true of course, in which case I assume they are randomly
% sampled.}

Fig.~\ref{fig:neg_size}  shows the effect of the negative sample size on the 
\MAX{} Loss function. We compare the caption retrieval performance for 
different negative set sizes varied from $2$ to $512$.  In practice, for 
negative set sizes smaller than the mini-batch size, $128$, we randomly sample 
the negative set from the mini-batch. In other cases where the mini-batch size 
is smaller than the negative set, we randomly sample the mini-batch from the 
negative set. We observe that on this dataset, the optimal negative set size is 
around $128$.  Interestingly, for negative sets as small as $2$, R@$1$ is 
slightly below \VSEz{}. To understand this, note that the \SUM{} loss is still 
over a large sample size which has a relatively high probability of containing 
hard negatives. For large negative sets, the model takes longer to train for 
the first epochs. Using the negative set size $512$, the performance dropped.  
This can be due to the small size of the dataset and the increase in the 
probability of sampling the hardest negative and outliers. Even though the 
performance drops with larger mini-batch sizes, it still performs better than 
the \SUM{} loss.



==> neg_size_table.tex <==
% f30k_vse0_vggfull_epoch5_vse0_neg128
rsum: $298.7$ &
Average i2t Recall: $54.2$ &
Image to text: $31.6$ & $59.3$ & $71.7$ & $4.0$ & $25.3$&
Average t2i Recall: $45.4$ &
Text to image: $21.6$ & $50.7$ & $63.8$ & $5.0$ & $30.0$

% f30k_vse0_vggfull_epoch5_vse++_neg128
rsum: $325.4$ &
Average i2t Recall: $58.5$ &
Image to text: $36.1$ & $63.8$ & $75.5$ & $3.0$ & $20.7$&
Average t2i Recall: $50.0$ &
Text to image: $27.0$ & $55.8$ & $67.2$ & $4.0$ & $29.6$

% f30k_vse0_vggfull_epoch5_vse++_neg2
rsum: $282.1$ &
Average i2t Recall: $50.4$ &
Image to text: $26.3$ & $56.2$ & $68.8$ & $4.0$ & $29.8$&
Average t2i Recall: $43.6$ &
Text to image: $20.6$ & $48.3$ & $61.9$ & $6.0$ & $30.8$

% f30k_vse0_vggfull_epoch5_vse++_neg64
rsum: $335.2$ &
Average i2t Recall: $60.8$ &
Image to text: $38.0$ & $67.1$ & $77.4$ & $2.0$ & $20.6$&
Average t2i Recall: $50.9$ &
Text to image: $27.5$ & $57.1$ & $68.2$ & $4.0$ & $28.3$

% f30k_vse0_vggfull_epoch5_vse++_neg512_X4_epoch50
rsum: $300.7$ &
Average i2t Recall: $54.3$ &
Image to text: $32.5$ & $58.8$ & $71.6$ & $3.0$ & $48.4$&
Average t2i Recall: $45.9$ &
Text to image: $24.6$ & $51.2$ & $62.0$ & $5.0$ & $41.0$

% f30k_vse0_vggfull_epoch5_vse++_neg32
rsum: $330.3$ & 
Average i2t Recall: $59.9$ &
Image to text: $36.6$ & $67.1$ & $76.0$ & $3.0$ & $21.7$&
Average t2i Recall: $50.2$ &
Text to image: $26.6$ & $56.1$ & $67.8$ & $4.0$ & $28.4$

% f30k_vse0_vggfull_epoch5_vse++_neg16
rsum: $320.9$ & 
Average i2t Recall: $57.9$ &
Image to text: $34.2$ & $64.1$ & $75.3$ & $3.0$ & $20.8$&
Average t2i Recall: $49.1$ &
Text to image: $25.3$ & $55.1$ & $66.9$ & $4.0$ & $28.0$

% f30k_vse0_vggfull_epoch5_vse++_neg8
rsum: $309.0$ & 
Average i2t Recall: $55.3$ &
Image to text: $31.5$ & $60.9$ & $73.5$ & $3.0$ & $22.8$&
Average t2i Recall: $47.7$ &
Text to image: $23.7$ & $53.6$ & $65.8$ & $5.0$ & $29.2$

% f30k_vse0_vggfull_epoch5_vse++_neg4
rsum: $298.6$ & 
Average i2t Recall: $53.5$ &
Image to text: $29.5$ & $59.0$ & $72.1$ & $4.0$ & $25.3$&
Average t2i Recall: $46.0$ &
Text to image: $22.0$ & $51.6$ & $64.4$ & $5.0$ & $29.2$

% f30k_vse0_vggfull
rsum: $301.8$ &
Average i2t Recall: $54.6$ &
Image to text: $31.2$ & $61.2$ & $71.5$ & $3.0$ & $23.5$&
Average t2i Recall: $46.0$ &
Text to image: $21.9$ & $51.5$ & $64.5$ & $5.0$ & $29.8$

% runs_extra/f30k_vse0_vggfull_epoch5_vse++_neg256_X2_epoch50
rsum: $315.4$ &
Average i2t Recall: $56.8$ &
Image to text: $34.6$ & $62.7$ & $73.2$ & $3.0$ & $31.2$&
Average t2i Recall: $48.3$ &
Text to image: $26.6$ & $53.8$ & $64.5$ & $4.0$ & $35.9$


==> spotlight.tex <==
%%%% 1
\section{Problem definition}
Here we focus on visual-semantic embeddings for cross-modal retrieval; i.e.\ 
the retrieval of images given captions, or of captions for a query image.  As 
is common in retrieval, we measure performance by R@$K$, i.e., recall at $K$ -- 
the fraction of queries for which the correct item is retrieved in the closest 
$K$ points to the query in the embedding space ($K$ is usually a small integer, 
often $1$).

%%%% 2
\section{Contribution}
Our main contribution is to incorporate hard negatives in the loss function for 
multi-modal embeddings.  Minimizing a loss function using hard negative mining 
is equivalent to minimizing a modified non-transparent loss function with 
uniform sampling.  We extend the idea with the explicit introduction of hard 
negatives in the loss function for multi-modal embeddings, without any 
additional cost of mining.

%%%% 3
\section{Intuitive Figure}
\input{max_vs_sum_fig}


\section{Formulation}
%%%%% 4
\subsection{SH}
\begin{equation}
    \ell_{SH}(i, c) ~=~
    \sum_{\hat{c}} [\alpha - s(i,c) + s(i,\hat{c})]_+ 
 \, +\, \sum_{\hat{i}} [\alpha - s(i,c) + s(\hat{i},c)]_+\,,
    \label{eq:contrastive}
\end{equation}

%%%%% 5
\subsection{MH}
\begin{equation}
    \ell_{MH}(i, c)
    ~=~ \max_{c^\prime} \left[\alpha + s(i,c^\prime) - s(i,c)\right]_+
    \, +\, \max_{i^\prime} \left[\alpha + s(i^\prime,c) -s(i,c)\right]_+ ~ .
    \label{eq:rank_loss}
\end{equation}

\section{Results}
%%% 6
\subsection{MS-COCO}
\begin{table*}[t!]
\input{results_table}
\end{table*}
%\bigskip

\subsection{Ablation study}
%%%% 7
\begin{table*}[t!]
\input{vse0_table}
\end{table*}

\section{Examples}
%%%% 8
\input{sample_hard_negatives_128}
%%%% 9
\input{sample_outputs}

